Pseudocylindrical Convolutions for Learned Omnidirectional Image Compression

Although equirectangular projection (ERP) is a convenient form to store omnidirectional images (also known as 360-degree images), it is neither equal-area nor conformal, thus not friendly to subsequent visual communication. In the context of image compression, ERP will over-sample and deform things and stuff near the poles, making it difficult for perceptually optimal bit allocation. In conventional 360-degree image compression, techniques such as region-wise packing and tiled representation are introduced to alleviate the over-sampling problem, achieving limited success. In this paper, we make one of the first attempts to learn deep neural networks for omnidirectional image compression. We first describe parametric pseudocylindrical representation as a generalization of common pseudocylindrical map projections. A computationally tractable greedy method is presented to determine the (sub)-optimal configuration of the pseudocylindrical representation in terms of a novel proxy objective for rate-distortion performance. We then propose pseudocylindrical convolutions for 360-degree image compression. Under reasonable constraints on the parametric representation, the pseudocylindrical convolution can be efficiently implemented by standard convolution with the so-called pseudocylindrical padding. To demonstrate the feasibility of our idea, we implement an end-to-end 360-degree image compression system, consisting of the learned pseudocylindrical representation, an analysis transform, a non-uniform quantizer, a synthesis transform, and an entropy model. Experimental results on $19,790$ omnidirectional images show that our method achieves consistently better rate-distortion performance than the competing methods. Moreover, the visual quality by our method is significantly improved for all images at all bitrates.

==> fig_neighbor.tex <==
\begin{figure}[tb!]
     %\centering
     \begin{minipage}{1\linewidth}
     \begin{minipage}{0.45\linewidth}
     \vspace{0.3cm}
     \begin{tikzpicture}
    	\node[inner sep=0pt] (nd1) at (0,0) {\includegraphics[width=1.\linewidth]{sample/plannar_sample.pdf}};
	 \end{tikzpicture}
     \end{minipage}
     \begin{minipage}{0.55\linewidth}
     \begin{tikzpicture}
    	\node[inner sep=0pt] (nd1) at (0,0) {\includegraphics[width=1.\linewidth]{sample/sphere_sample.pdf}};
		\draw [line width=0.15mm] (0.9,1.04) -- (1.7,1.04);
		\node[text width=3cm,align=center] (cp10) at (1.9,1.04){\baselineskip=3pt \scriptsize{$\delta_{\phi}$} \par};
		\draw [line width=0.15mm] (0.95,0.4) -- (1.7,0.4);
		\node[text width=3cm,align=center] (cp11) at (1.9,0.4){\baselineskip=3pt \scriptsize{$\delta_{\theta}$} \par};
		\node[text width=3cm,align=center] (cp11) at (-0.9,1.9){\baselineskip=3pt \scriptsize{$\phi_q$} \par};
		\node[text width=3cm,align=center] (cp11) at (1.2,2.3){\baselineskip=3pt \scriptsize{$\phi_q  + \pi$} \par};
	 \end{tikzpicture}
     \end{minipage}
     \end{minipage}
     \begin{minipage}{1\linewidth}
     \begin{minipage}{0.45\linewidth}
     \center{\scriptsize{(a)}}
     \end{minipage}
     \begin{minipage}{0.55\linewidth}
     \center{\scriptsize{(b)}}
     \end{minipage}
     \end{minipage}
     
     \caption{Illustration of the neighborhood in the (a) planar and (b) spherical representation.}
     \label{fig:neighbor}
 \end{figure}
